Two Trades is not Baffled: Condensing Graph via Crafting Rational Gradient Matching

Training on large-scale graphs has achieved remarkable results in graph representation learning, but its cost and storage have raised growing concerns. As one of the most promising directions, graph condensation methods address these issues by employing gradient matching, aiming to condense the full graph into a more concise yet information-rich synthetic set. Though encouraging, these strategies primarily emphasize matching directions of the gradients, which leads to deviations in the training trajectories. Such deviations are further magnified by the differences between the condensation and evaluation phases, culminating in accumulated errors, which detrimentally affect the performance of the condensed graphs. In light of this, we propose a novel graph condensation method named \textbf{C}raf\textbf{T}ing \textbf{R}ationa\textbf{L} trajectory (\textbf{CTRL}), which offers an optimized starting point closer to the original dataset's feature distribution and a more refined strategy for gradient matching. Theoretically, CTRL can effectively neutralize the impact of accumulated errors on the performance of condensed graphs. We provide extensive experiments on various graph datasets and downstream tasks to support the effectiveness of CTRL. Code is released at https://github.com/NUS-HPC-AI-Lab/CTRL.

==> 6.ImpactStatements.tex <==
\section{Impact Statements} \label{Impact Statements}
\textbf{Ethical impacts.} We assure you that our paper has no ethical concerns, including its motivation, designs, experiments, and the data used. The proposed CTRL aims to further improve the field of graph condensation.

\textbf{Expected societal implications.}
Performing GNN training on actual graph data incurs a significant computational expense. Graph condensation provides a more efficient way of computation by reducing the size of the graph data. This reduction in size helps to diminish the energy consumption of computing devices, thereby decreasing carbon emissions. Such a reduction in carbon emissions is extremely beneficial to the environment and contributes to sustainability efforts.

==> tables/NAS.tex <==
\begin{table*}
  \centering
  \scriptsize
  \caption{Neural Architecture Search. Methods are compared in validation accuracy correlation and test accuracy obtained by searched architecture. Whole means the architecture is searched using whole dataset.}
  \label{tab:cross}
  \fontsize{7}{11}\selectfont
   \begin{tabularx}{\linewidth}{*{5}{>{\centering\arraybackslash}X}|*{5}{>{\centering\arraybackslash}X}}
    \toprule
     & \multicolumn{4}{c}{ Pearson Correlation} & \multicolumn{5}{c}{Test Accuracy} \\
     \midrule
     &Random&Herding&GCond&CTRL&Random&Herding&GCond&CTRL&Whole\\
     \midrule
    Cora & 0.40 & 0.21 & 0.76 & 0.86 & 82.9 & 82.9 & 83.1 & 83.2 & 82.6 \\
    Citeseer & 0.56 & 0.29 & 0.79 & 0.93 & 71.4 & 71.3 & 71.3 & 72.0 &71.6 \\
    Pubmed & 0.55 & 0.21 & 0.81 & 0.83 & 80.0 & 79.9 & 79.7 & 80.1 & 80.5 \\
    \bottomrule
  \label{tab:NAS}%
\end{tabularx}
\end{table*}


==> tables/ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\vspace{-1mm}
\caption{Ablation studies of learning objectives and MTN on Office-Home.}\label{tab:ablation}
\scriptsize
\resizebox{\columnwidth}{!}{
    \begin{tabular}{
    ccccc|cccccc
    >{\columncolor[HTML]{DAE8FC}}c}
    \toprule
    $\mathcal{L}_{dd}$ & $\mathcal{L}_{kd}$ & $\mathcal{L}_{mi}$ & $\mathcal{L}_{adv}$ & MTN          & Ar$\to$Cl & Cl$\to$Ar & Cl$\to$Pr & Pr$\to$Ar & Pr$\to$Cl & Re$\to$Cl & H. Avg. \\ \midrule
                       &                    &                    &                                       &              & 44.1  & 54.5  & 63.3  & 52.8  & 41.2  & 46.7  & 50.4    \\
    $\checkmark$       &                    &                    &                                       &              & 55.5  & 65.4  & 76.5  & 64.4  & 50.7  & 58.1  & 61.8    \\
    & $\checkmark$       &                    &                                       &              & 54.6  & 63.8  & 75.3  & 62.3  & 48.0    & 55.7  & 60.0    \\
    $\checkmark$       &                    &                    &                                       & $\checkmark$ & 56.6  & 65.0    & 76.7  & 64.1  & 51.6  & 60.4  & 62.4    \\
    $\checkmark$       &                    & $\checkmark$       &                                       & $\checkmark$ & 55.4  & 67.6  & 78.4  & 65.4  & 54.5  & 58.5  & 63.3    \\
    $\checkmark$       & $\checkmark$       & $\checkmark$       &                                       & $\checkmark$ & 56.8  & 68.1  & 78.7  & 67.3  & 55.3  & 59.2  & 64.2    \\
    $\checkmark$       & $\checkmark$       & $\checkmark$       & $\checkmark$                          & $\checkmark$ & 57.2  & 68.0  & 78.6  & 67.5  & 56.0  & 58.9  & 64.4   \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-3mm}
\end{table*}
